The Challenge of Crafting Intelligible Intelligence

Since Artificial Intelligence (AI) software uses techniques like deep lookahead search and stochastic optimization of huge neural networks to fit mammoth datasets, it often results in complex behavior that is difficult for people to understand. Yet organizations are deploying AI algorithms in many mission-critical settings. To trust their behavior, we must make AI intelligible, either by using inherently interpretable models or by developing new methods for explaining and controlling otherwise overwhelmingly complex decisions using local approximation, vocabulary alignment, and interactive explanation. This paper argues that intelligibility is essential, surveys recent work on building such systems, and highlights key directions for research.

==> 8-notes.tex <==
Terminology:

intelligible  *
interpretable  *
blackbox
opaque
inscrutable  *
explanation
understandable
transparent
trust



==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> old-1-intro.tex <==
to do
* check miller - https://arxiv.org/pdf/1706.07269.pdf insights from SS
* check simple vs likely - Lombrozo Simplicity and probability in causal explanation
* check GAM algorithms



\section{Introduction}





Rationale - Key to trustworthy AI
* Good expl -- establishes trust, which means that a user can predict system's behavior 
* legal / ethical issues as AI adopted socially (Recitivism) - fairness papers
* AI safety +  learned utility models
* XAI vs XML

Ai systems increasingly deployed and used in mission critical roles

Unlike other mission critical software, it’s very hard to test AI. systems very complex.  Decisions are context specific. Millions of factors involved. almost by defn there is no deterministic method for accomplishing the AI’s task

So ability for AI system to explain its reasoning is crucial for users to be sure that the AI is trustworthy.
G
generating good explanations is at intersection of AI \& HCI



\subsection{History}



 
* philosophy - Hempel - two types of explanation,  'deductive-nomological' (DN) and 'inductive-statistical' (IS). 
Start with initial conditions, use rules (laws) to conclude the thing to be explained. Difference between DN an IS is nature of the rules.  DN rules are logical universals. IS are 'almost always'

Criticisms - relevance and asymmetry (lack of preference wrt causality)

Salmon - aim is scientfic understanding.
 causal theory of explanation 
 
 "At this point, fundamental disagreements on the nature of explanation fall into one of two categories. First, there are metaphysical disagreements. Realists and anti-realists continue to differ over what sort of ontological commitments one makes in accepting an explanation. Second, there are meta-philosophical disagreements. Naturalists and non-naturalists remain at odds concerning the relevance of scientific inquiry ( namely, inquiry into the way scientists, ordinary people and computers actually think) to a philosophical theory of explanation. " Fortunately, none of this matters.\footnote{http://www.iep.utm.edu/explanat}


early expert systems - \cite{shortliffe-inexact75} motivated the importance of expert systems explaining their reasoning.
\cite{swartout-xplain83} presents an early explainer. User study to determine what kinds of questions doctors would ask. Noted justifications were sought: simple trace is insufficient; also need  justifications for why decisions are ok.  Uses background theory to synthesize these explanations.  


* recommender systems
Herlocker et al 200 - measuered user satisfaction with different explaianitions - simple and conclusive.

Papadimitrious et al\footnote{A. Papadimitriou, P. Symeonidis,
and Y. Manolopoulos. A generalized taxonomy of
explanations styles for traditional and social recommender
systems. Data Min. Knowl. Discov., 24(3):555–583, 2012.} - classifier rec system explanations into three types: 1) based on user's previous choices, 2) based on the ratings fo similar users, 3) based on features. Showe dthat a hybrid method worked best

Bilgic and mooney 2005\footnote{Explaining recommendations: Satisfaction vs.
promotion. In Workshop on the Next Stage of Recommender
Systems Research, San Diego, CA, 2005} distibnguish between persuasiveness and justifiability of explanations - argue feature based methods are most justifiable.


\subsection{Desiderata for good explanations}

* Interpretable - a function of a user’s background knowledge
* Local fidelity
* Global perspective
* model-agnostic
* actionable - let's user know they can trust system, ask follow up questions if unsure, or change things if they suspect system is wrong.
* Transparency: How many assumptions does the explainer fail to communicate? Lower is better.

Lombrozo 2007 shows that humans prefer explanations that are
* simpler (fewer clauses)  - more important than "likely" - TBD what does this mean?  
* more general
* coherent - consistent with prior beliefs
key objective: listener understands and accepts explanation. (But is it better to give a simple, incorrect explanation that the user accepts or a faithful one?

People explain things for all sorts of different reasons --- explanation as communication act - what is the explainer's intent?

Extrinsic evaluation methods:
* Strengths and Limitations: 
  ** Does it enable the user to find issues with the system or predict future behavior [marco, anchor]? 
  ** Detect anomalies/UUs [Marco, Bansal]; determine if it is right for the wrong reasons [Marco]; 
  ** craft adversarial examples [Percy]
* Debugging; 
  ** Does it enable the user to fix the system? Provide supervision [Percy, Ross]; 
  ** perform model selection [Marco]; 
  ** fix mislabeled examples [Percy] Amershi



Challenges
* Complexity / approximation tradeoff (fidelity / interpretability)
  This comes up in terms of the complexity of the hypothesis, and …
  Also in the underlying vocbulary - eg pixels in gradient methods and super pixels in LIME
* Per prediction or overall explanation?  ( Local / global)
* Black box / model-specific
* Audience: background, intent, dialog
* Dialog + drilldown
* Vocabulary, features, subconcepts - disjunction
   LIME uses pipeline - segment image using black box system that knows nothing about example or prediction or hidden    layers or classifier. Can’t possibly be right.
   Vocabulary is learned by hidden layers
   Really wish to expose high-level features.  Eg topology for digit recognition, not individual pixels.
   
Challenges / Observations fro Miller
* explanations are contrastive Q "why did joe open the window?" A = "because he was hot" assumes vs not open window? vs turn on AC? vs asking helen to open window?
* attribution theory and explanation selection - how choose what NOT to say
   social vs causal attribution?  BDI theory. different explns for success vs failure
   choice of causal sources - which events to undo: proximal (ds distant). abnormal (vs normal), controllable
* explanation is an interactive conversation.  [hilton 1990?]
   Grice's maxims guide conversation
   * quality (only say what you mean)
   * quality (only say as much as necessary)
   * relation (only say what is relevant)
   * manner (say it nicely)

Moderately complex learning problesm - use linear or GAMs
* Works well for moderate number of ordinal variables where features have meaning
   ** Doesn’t add much for Boolean variables
   ** Check to see what they do with nominal variables
* Linearity: Quick and easy for domain expert to double check (and gain insight) from model
* Examples: Rich Caruana – effects correlated with hidden variable (has-asthma, has-heart-disease…, age=65
  Social effects – age = 85, age = 100
  Feedback from treatment – creatine >5, >10

-----------------------------
connection to bias and UUs

Bias examples: iraqi tank, turkish translation, 
    
UnkUnk -> bias (ece examples); training RL on simulator

----------

Evaluating Explanatory Dialog
* Automatic Methods
* User Studies
  ** How many follow up questions do users ask? What different types of questions? How many can the system support?
  ** Bad: recover features in sparse model
  ** Can user predict what classifier will do on new test examples?
  ** Given a biased training set, can user predict what will happen on new examples
  ** How continuous/stable are the explanations: Given very similar inputs see if the explanation changes a lot? May be useful for verifying conjectures
  ** How fast the prediction changes as the parts of explanations are removed (features or training data)?

Previous work has adopted both automated metrics and user studies for evaluating their system. We will implement these existing methods and design new users studies for assessing the effectiveness of explanatory dialogs. Existing methods include evaluating explainer-model faithfulness \cite{Ribeiro2016}, representation interpretability \cite{Ribeiro2016}, and user’s effectiveness at tasks such as model selection \cite{Ribeiro2016}, debugging training data \cite{koh-icml1}, providing supervision \cite{koh-icml1, ross-gradient17}, and crafting adversarial examples \cite{koh-icml1}. The interactive nature of explanatory dialog also requires that we design new user studies that evaluate the number and nature of follow-up questions asked by the users, system’s ability to answer them, user’s understanding of the future behavior and finally, user productivity \& preference. As an example for evaluating if user can predict the model’s future behavior one can use a biased training set and evaluate the user’s ability to predict the model’s behavior on a held-out test set.





==> weld-defns-edited.tex <==
\newcommand{\comment}[1]{} 
\newcommand{\NOTE}[1]{\marginpar{\em {#1}}}
\newcommand{\bug}
    {\mbox{\rule{2mm}{2mm}}}
\newcommand{\Bug}[1]
    {\bug \footnote{BUG: {#1}}}
\newcommand{\QED}{\mbox{$\Box$}}
\newcommand{\ddt}{\mbox{$\frac{d}{dt}\,$}}  %* no strut

\newcommand{\etal}{\mbox{\it et al.}}
\newcommand{\etc}{\mbox{\it etc.}}
\newcommand{\eg}{\mbox{\it e.g.}}
\newcommand{\ie}{\mbox{\it i.e.}}
\newcommand{\cf}{\mbox{\it cf.}}
\newcommand{\Eg}{\mbox{\it E.g.}}
\newcommand{\Ie}{\mbox{\it I.e.}}
\newcommand{\?}{\mbox{?}}




\newcommand{\DEFN}{\mbox{$\stackrel{\mbox{\tiny def}}{=}$}}

\newcommand{\TT}[1]{\mbox{\tt #1}}
%\newcommand{\bi}{\begin{itemize}}
%\newcommand{\ei}{\end{itemize}}
\newcommand{\bi}{\begin{list}{$\bullet$}{
    \setlength{\leftmargin}{1.5 em}
    \setlength{\itemsep}{0 pt}
    \setlength{\topsep}{3 pt}
    \setlength{\parsep}{3 pt}
    \setlength{\partopsep}{0 pt}
    \setlength{\labelwidth}{1 em}
    \setlength{\labelsep}{0.5 em}
    \setlength{\parskip}{0cm}  }}
\newcommand{\ei}{\end{list}}

\newcommand{\BE}{\begin{enumerate}}
\newcommand{\EE}{\end{enumerate}}

%\newtheorem{defnctr}{Definition}
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}        
%\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{propos}[theorem]{Proposition}
%\newcommand{\proof}
%	{\vspace{-8pt}
%	 {\bf Proof:}}



\newcommand{\tuple}[1]
        {\mbox{$\langle{#1}\rangle$}}
\newcommand{\set}[1]
        {\mbox{$\{{#1}\}$}}
\newcommand{\size}[1]{\mbox{$\mid\!#1\!\mid$}}



\newcommand{\PROOF}[1]{\mbox{\noindent \proofbegin {#1} \proofend}}
\newcommand{\proofbegin}{\mbox{\bf Proof: \ }}
\newcommand{\proofend}{\Math{\Box}}
\newcommand{\st}{\mbox{ such that }}
\newcommand{\wht}{\mbox{ we have that }}
\newcommand{\entails}{\mbox{$\models$}}
\newcommand{\yields}{\mbox{$\models$}}
\newcommand{\dgets}{\mbox{$\leftarrow$}}

%\renewcommand{\baselinestretch}{0.985}




\newcommand{\initab}{                           % set up tab stops
\begin{tabbing}
XXX \= XXXX \= \kill
}
\newcommand{\begpub}{
\begin{quotation}
\noindent
}
\newcommand{\nextpub}{

\vspace{2mm}
\noindent
}
\newcommand{\finpub}{
\end{quotation}
}



\hyphenation{non-de-ter-mi-nis-tic-al-ly non-de-ter-mi-nis-tic
exis-ten-tial-ly quan-tified se-lec-tion exis-ting in-stan-tiated
uni-vers-al-ly es-tab-lish in-con-sis-tent}


% \newcommand{\ncd}{\mbox{$\neq$}}
% \newcommand{\cd}{\mbox{$=$}}
% \newcommand{\fabian}{\mbox{\sc fabian}}
% \newcommand{\occam}{\mbox{\sc occam}}
% \newcommand{\sadl}{\mbox{\sc sadl}}
% \newcommand{\socrates}{\mbox{\sc socrates}}
% \newcommand{\uwl}{\mbox{\sc uwl}}
% \newcommand{\spa}{\mbox{\sc spa}}
% \newcommand{\scr}{\mbox{\sc scr}}
% \newcommand{\strips}{\mbox{\sc strips}}
% \newcommand{\snlp}{\mbox{\sc snlp}}
% \newcommand{\cbur}{\mbox{\sc C-buridan}}
% \newcommand{\buridan}{\mbox{\sc buridan}}
% \newcommand{\xii}{\mbox{\sc xii}}
% \newcommand{\zeno}{\mbox{\sc zeno}}
% \newcommand{\adl}{\mbox{\sc adl}}
% \newcommand{\kr}{\mbox{\tt /kr94}}
% \newcommand{\ucpop}{\mbox{\sc ucpop}}
% 
% \newcommand{\cause}{{\tt cause}}
% \newcommand{\observe}{{\tt observe}}
% \newcommand{\satisfy}{{\tt satisfy}}
% \newcommand{\handsoff}{{\tt hands-off}}
% \newcommand{\findout}{{\tt find-out}}
% 
% \newcommand{\CAUS}{\mbox{C}}
% \newcommand{\OBS}{\mbox{O}}
% \newcommand{\PAT}{\mbox{\sf E}}
% \newcommand{\fact}{\mbox{$\varphi$}}
% \newcommand{\LIT}{\mbox{\sf p}}
% \newcommand{\lit}{\mbox{\LIT}}
% \newcommand{\litp}{\mbox{\LIT$^\prime$}}
% \newcommand{\rel}{\mbox{REL}}
% \newcommand{\change}[3]{\mbox{$\Delta(#1,{\tt #2}\rightarrow {\tt #3})$}}   
% 
% \newcommand{\true}{{\tt T}}
% \newcommand{\false}{{\tt F}}
% \newcommand{\unknown}{{\tt U}}
% 
%
